SLIM: A Well-Conditioned Single-Source Boundary Element Method for Modeling Lossy Conductors in Layered Media

The boundary element method (BEM) enables the efficient electromagnetic modelling of lossy conductors with a surface-based discretization. Existing BEM techniques for conductor modelling require either expensive dual basis functions or the use of both single- and double-layer potential operators to obtain a well-conditioned system matrix. The associated computational cost is particularly significant when conductors are embedded in stratified media, and the expensive multilayer Green's function (MGF) must be invoked. In this work, a novel single-source BEM formulation is proposed, which leads to a well-conditioned system matrix without the need for dual basis functions. The proposed single-layer impedance matrix (SLIM) formulation does not require the double-layer potential to model the background medium, which reduces the cost associated with the MGF. The accuracy and efficiency of the proposed method is demonstrated through realistic examples drawn from different applications.

==> figures/geom.tex <==
% \begin{tikzpicture}[scale = 0.7, >=latex]
%   %	\draw[black, fill = black!10] (-2,-1.5) rectangle (2,1.5);
%   %	\draw[black, fill = black!20] (-2,-2.5) rectangle (2,-1.5);
%   %	\draw[black, fill = black!20] (-2,1.5) rectangle (2,2.5);
%   \draw[black, fill = black!10] (0,0) ellipse (3.0cm and 1.8cm);
%   \draw[black, dashed, fill = none] (0,0) ellipse (2.9cm and 1.7cm);
%   \draw[black, dashed, fill = none] (0,0) ellipse (3.1cm and 1.9cm);
%   \node at (3.0, 0.2) [right] {$\mathcal{S}_i^+$};
%   \node at (2.9, 0.2) [left] {$\mathcal{S}_i^-$};
%   % 
%   \draw[black, ->, line width = 0.4mm] (0, -1.8) -- (0, -2.4);
%   \node at (0, -2.4) [right] {${\nhat}_i$};
%   % 
%   \draw[black, ->, line width = 0.4mm] (0, 1.8) -- (0, 1.2);
%   \node at (0, 1.2) [right] {${\nhat}_0$};
%   % 
%   \node at (0.0,-0.7) {$({\mu_i}, {\epsilon_i}, \sigma_i)$};
%   \node at (0.0,0.4) [below] {$\vect{E}_i(\vect{r}), \vect{H}_i(\vect{r})$};
%   % 
%   \node at (-1.4,0.8) [left]{${\mathcal{V}_i}$};
%   % 
%   \draw[black, thick] (-3.0cm,0.0cm)--+(0.4,0);
%   \node at (-2.0,0.0) [left]{${\mathcal{S}_i}$};
%   % 
%   %	\draw[dashed, path fading = west] (0.35, -1.8) arc(-85:85:3.0cm and 1.8cm);
%   %	\node at (3.0, 0.2) [right] {$\mathcal{S}_i^+$};
%   %	\draw[dashed, path fading = west] (0.18, -1.8) arc(-85:85:3.0cm and 1.8cm);
%   %	\node at (2.9, 0.2) [left] {$\mathcal{S}_i^-$};
%   % 
%   \node at (-3.0,1.1) [left]{${\mathcal{V}_0}$};
%   % 
%   \node at (-3,-1.4) [below] {$\vect{E}_0(\vect{r}), \vect{H}_0(\vect{r})$};
%   \node at (-3, -2.5) {$(\mu_0,\epsilon_0)$};
%   % 
%   \node at (-2.6,3.2) [below] {$\vect{E}_\mathrm{inc}(\vect{r}), \vect{H}_\mathrm{inc}(\vect{r})$};
%   \draw[->,thick, black] (-3.0, 2.3)--+(0.6, -0.6);
%   \draw[thick, black] (-2.8, 1.9)--+(0.2, 0.2);
%   \draw[thick, black] (-2.9, 2.0)--+(0.2, 0.2);
%   % 
%   %	\node at (-0.9, -2.1) {$(\mu_{l+1},\epsilon_{l+1})$};
%   %	\node at (-0.9, 2.1) {$(\mu_{l-1},\epsilon_{l-1})$};
%   %	\node at (1.2, -1.1) {layer $l$};
%   %	\node at (1.2, -2.1) {layer $l+1$};
%   %	\node at (1.2, 2.1) {layer $l-1$};
% \end{tikzpicture}

\begin{tikzpicture}[scale = 0.7, >=latex]
  %	\draw[black, fill = black!10] (-2,-1.5) rectangle (2,1.5);
  %	\draw[black, fill = black!20] (-2,-2.5) rectangle (2,-1.5);
  %	\draw[black, fill = black!20] (-2,1.5) rectangle (2,2.5);
  \draw[black, fill = black!10] (0,0) ellipse (3.0cm and 1.8cm);
  \draw[black, dashed, fill = none] (0,0) ellipse (2.9cm and 1.7cm);
  \draw[black, dashed, fill = none] (0,0) ellipse (3.1cm and 1.9cm);
  \node at (3.0, 0.2) [right] {$\mathcal{S}^+$};
  \node at (2.9, 0.2) [left] {$\mathcal{S}^-$};
  % 
  \draw[black, ->, line width = 0.4mm] (0, -1.8) -- (0, -2.4);
  \node at (0, -2.4) [right] {${\nhat}$};
  % 
  \draw[black, ->, line width = 0.4mm] (0, 1.8) -- (0, 1.2);
  \node at (0, 1.2) [right] {${\nhat}_0$};
  % 
  \node at (0.0,-0.7) {$({\mu}, {\epsilon}, \sigma)$};
  \node at (0.0,0.4) [below] {$\vect{E}(\vect{r}), \vect{H}(\vect{r})$};
  % 
  \node at (-1.4,0.8) [left]{${\mathcal{V}}$};
  % 
  \draw[black, thick] (-3.0cm,0.0cm)--+(0.4,0);
  \node at (-2.0,0.0) [left]{${\mathcal{S}}$};
  % 
  %	\draw[dashed, path fading = west] (0.35, -1.8) arc(-85:85:3.0cm and 1.8cm);
  %	\node at (3.0, 0.2) [right] {$\mathcal{S}_i^+$};
  %	\draw[dashed, path fading = west] (0.18, -1.8) arc(-85:85:3.0cm and 1.8cm);
  %	\node at (2.9, 0.2) [left] {$\mathcal{S}_i^-$};
  % 
  \node at (-3.0,1.1) [left]{${\mathcal{V}_l}$};
  % 
  % \node at (-3,-1.4) [below] {$\vect{E}_0(\vect{r}), \vect{H}_0(\vect{r})$};
  \node at (-3, -2.5) {$(\mu_l,\epsilon_l)$};
  % 
  \node at (-2.6,3.2) [below] {$\vect{E}_\mathrm{inc}(\vect{r}), \vect{H}_\mathrm{inc}(\vect{r})$};
  \draw[->,thick, black] (-3.0, 2.3)--+(0.6, -0.6);
  \draw[thick, black] (-2.8, 1.9)--+(0.2, 0.2);
  \draw[thick, black] (-2.9, 2.0)--+(0.2, 0.2);
  % 
  %	\node at (-0.9, -2.1) {$(\mu_{l+1},\epsilon_{l+1})$};
  %	\node at (-0.9, 2.1) {$(\mu_{l-1},\epsilon_{l-1})$};
  %	\node at (1.2, -1.1) {layer $l$};
  %	\node at (1.2, -2.1) {layer $l+1$};
  %	\node at (1.2, 2.1) {layer $l-1$};
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../jnl-2020-awpl-SLIM"
%%% End:

